Background ambiguity and the G\"odel double copy

In this work, we investigate the assumptions regarding spacetime backgrounds underlying the classical double copy. We argue (contrary to the norm) that single-copy fields naturally constructed on the original curved background metric are only interpretable on a flat metric when such a well-defined limit exists, for which Kerr--Schild coordinates offer a natural choice. As an explicit example where such a distinction matters, we initiate an exploration of single-copies for the G\"odel universe. This metric lacks a (geodesic) Kerr--Schild representation yet is Petrov type-D, meaning the technology of the ``Weyl double copy" may be utilized. The Weyl derived single copy has many desirable features, including matching the defining properties of the spacetime, and being sourced by the mixed Ricci tensor just as Kerr--Schild single copies are. To compare, we propose a sourced flat-space single-copy interpretation for the G\"odel metric by leveraging its symmetries, and find that this proposal lacks the defining properties of the spacetime, and is not consistent with the flat limit of our curved-space single copy. Notably, this inconsistency does not occur in Kerr--Schild metrics. Our curved-space single copy also lead to the same electromagnetic analogue of the G\"odel universe found separately through tidal force analogies, opening a new avenue of exploration between the double copy and gravitoelectromagnetism programs.

==> figs/orderOfOperations.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[yscale=0.65]
\node (dc1) at (0,1) {Cyl. G\"odel \eqref{godelMetricCyl}};
\node (dc2) at (5,1) {Planar G\"odel \eqref{godelmetric}};

\node (a) at (11,0) {Flat indices};

\node (sc1) at (5,-1) {Planar flat \eqref{backgroundPlanar}};
\node (sc2) at (0,-1) {Cyl. flat \eqref{cylBackground}};

\draw[<->] (dc1) -- node[above]{\footnotesize{coords.}} (dc2);
\draw[<->] (sc1) -- node[below]{\footnotesize{coords.}} (sc2);

\draw[<->] (dc2) -- node[above,rotate=-6.183]{\footnotesize{tetrad \eqref{cplxg1}--\eqref{cplxg3}}} (a);
\draw[<->] (sc1) -- node[below,rotate=6.183]{\footnotesize{tetrad ($\omega \to 0$)}} (a);

\end{tikzpicture}
\caption{A flowchart showing the relationships between different coordinates in our study of the G\"odel metric. We want to study the single-copy fields on flat space in cylindrical coordinates \eqref{cylBackground}, but we have actually constructed the Weyl spinor from a null tetrad encoding the metric in planar coordinates \eqref{godelmetric}. Thus we need to first construct the single-copy gauge fields with the $\omega \to 0$ limit of the planar metric \eqref{backgroundPlanar} as our background spacetime. Then, we can apply a coordinate transformation [found by taking $\omega \to 0$ in \eqref{coordcyl1}--\eqref{coordcyl3}] to get back to cylindrical coordinates \eqref{cylBackground}.}
\label{figs:orderOfOperations}
\end{figure}
